Let Occ Flow: Self-Supervised 3D Occupancy Flow Prediction

Accurate perception of the dynamic environment is a fundamental task for autonomous driving and robot systems. This paper introduces Let Occ Flow, the first self-supervised work for joint 3D occupancy and occupancy flow prediction using only camera inputs, eliminating the need for 3D annotations. Utilizing TPV for unified scene representation and deformable attention layers for feature aggregation, our approach incorporates a novel attention-based temporal fusion module to capture dynamic object dependencies, followed by a 3D refine module for fine-gained volumetric representation. Besides, our method extends differentiable rendering to 3D volumetric flow fields, leveraging zero-shot 2D segmentation and optical flow cues for dynamic decomposition and motion optimization. Extensive experiments on nuScenes and KITTI datasets demonstrate the competitive performance of our approach over prior state-of-the-art methods. Our project page is available at https://eliliu2233.github.io/letoccflow/

==> content.tex <==

% 段落间距
\setlength{\parskip}{.24em}

\begin{abstract}
    % 王老师修改意见：
    % intro:
    % 1. para1:直接讲occflow，减少det和occ的描述
    % 2. para2:现有occflow依赖3D annotation,static occupancy自监督方法的出现，提出flow能否self-supervise
    % 3. our method提一下目前2d model的泛化性强（sam），flow可以通过self-supervise泛化
    % 4. contribution第二点提一下两阶段训练等优化策略
    % method
    % 1. selfocc相同的部分放suppl(neus render等)
    % 2. flow监督部分提一下同时提高静态和动态效果 (highlight)
    % result:
    % 1. 对比方法结果提供discuss，为什么我们的方法更好
    % 2. nuscenes对比方法？(selfocc,occnerf)
    % Accurate perception of the surrounding environment is crucial for autonomous driving systems and robotics. This paper introduces Let Occ Flow, the first self-supervised method for joint 3D occupancy and occupancy flow prediction using only camera inputs, eliminating the need for 3D annotations. Utilizing Tri-perspective View (TPV) for unified scene representation and deformable attention layers for feature aggregation, our approach incorporates a backward-forward temporal attention module to capture dynamic object dependencies. A resnet-like\yx{Is that okay? (I'm not sure)} 3D encoder and deconvolution module refine the volumetric scene representation. Our method extends differentiable rendering to 3D volumetric flow fields, leveraging 2D segmentation and optical flow modules for dynamic decomposition and optimization. Extensive experiments on nuScenes and KITTI datasets demonstrate the competitive performance of our approach.
    Accurate perception of the dynamic environment is a fundamental task for autonomous driving and robot systems. This paper introduces Let Occ Flow, the first self-supervised work for joint 3D occupancy and occupancy flow prediction using only camera inputs, eliminating the need for 3D annotations. Utilizing TPV for unified scene representation and deformable attention layers for feature aggregation, our approach incorporates a backward-forward temporal attention module to capture dynamic object dependencies, followed by a 3D refine module for fine-gained volumetric representation. Besides, our method extends differentiable rendering to 3D volumetric flow fields, leveraging zero-shot 2D segmentation and optical flow cues for dynamic decomposition and motion optimization. Extensive experiments on nuScenes and KITTI datasets demonstrate the competitive performance of our approach over prior state-of-the-art methods.
\end{abstract}

% Two or three meaningful keywords should be added here
\keywords{3D occupancy prediction, occupancy flow, Neural Radiance Field} 
%===============================================================================

\section{Introduction}

Accurate perception of the surrounding environment is crucial in autonomous driving and robotics for downstream planning and action decisions. Recently, vision-based 3D object detection~\citep{bevformer, bevdepth} and occupancy prediction~\citep{surroundocc, simpleocc, occnerf, selfocc, renderocc} have garnered significant attention due to their cost-effectiveness and robust capabilities. Building on these foundations, the concept of occupancy flow prediction has emerged to offer a comprehensive understanding of the dynamic environment by estimating the scene geometry and object motion within a unified framework~\citep{occnet, viewformer}.

%Though 3D object detection offers precise perception of the position and velocity of foreground objects, it faces challenges with long-tail problems and is prone to failure when encountering unexpected categories in real-world scenarios, posing potential safety hazards in practical applications. In contrast, occupancy prediction decouples geometry and semantics, delivering a more detailed perception of real scenes with irregular objects and unlabeled categories. Despite offering fine-grained geometry perception, occupancy prediction cannot offer motion information about the dynamic environment, which is crucial for planning and decision-making.
% Despite the strong performance of vision-based perception methods, most existing techniques rely on comprehensive 3D annotations, making them challenging to apply to large-scale training data. Some approaches have attempted to leverage LiDAR measurements to automatically create occupancy annotations~\citep{surroundocc, occbev, tpvformer}, but struggle to balance accuracy and completeness due to the inherent sparsity of LiDAR data and the presence of dynamic objects. Recently some methods have been proposed to provide accurate 3D occupancy prediction in a self-supervised manner by incorporating the NeRF-style differentiable rendering principle with weak 2D depth~\citep{renderocc} or photometric supervision~\citep{occnerf, selfocc}. 

Existing occupancy flow prediciton methods~\citep{occnet, viewformer} rely heavily on detailed 3D occupancy flow annotations, which complicates their scalability to extensive training datasets. Previous research has attempted to address the dependency on 3D annotations for occupancy prediction tasks. Some strategies utilized LiDAR data to generate occupancy labels~\citep{surroundocc, occbev, tpvformer}, but struggle to balance between accuracy and completeness due to LiDAR's inherent sparsity and dynamic object movements. 
Recently, some methods have emerged to enable 3D occupancy predictions in a self-supervised manner by integrating the NeRF-style differentiable rendering with either weak 2D depth cues~\citep{renderocc} or photometric supervision~\citep{occnerf, selfocc}.
However, existing self-supervised techniques take static world assumption as a premise and never consider the motion of foreground objects. This raises a question: \textit{Can we bridge 2D perception cues to enable self-supervised occupancy flow prediction?}
%Consequently, current occupancy flow prediction methods still rely on complete 3D occupancy and occupancy flow annotations, which are extremely challenging and expensive to obtain through semi-automatic or manual annotation.

To address the aforementioned issues, we introduce Let Occ Flow, a novel method for simultaneously predicting 3D occupancy and occupancy flow using only camera input, without requiring any 3D annotations for supervision, as shown in Figure~\ref{fig:teaser}. Our approach employs Tri-perspective View(TPV)~\citep{tpvformer} as a unified scene representation and incorporates deformable attention layers to aggregate multi-view image features. For temporal sequence inputs, we utilize a BEV-based backward-forward attention module to effectively capture long-distance dependencies of dynamic objects. Subsequently, we use a 3D refine module for spatial volume feature aggregation and transform the scene representation into fine-grained volumetric fields of SDF and flow. 

Differentiable rendering techniques are then applied to jointly optimize scene geometry and object motion.  Specifically, for geometry optimization, we employ a photometric consistency supervision~\citep{selfocc}. While LiDAR data is available, we employ range rendering supervision~\citep{unisim, emernerf} for efficient geometric-aware sampling and avoiding the occlusion caused by the extrinsic parameters between LiDAR and the camera sensors. 
For motion optimization, we leverage semantic and optical flow cues for dynamic decomposition and supervision. These cues are convenient to obtain from pre-trained 2D models, which have shown superior zero-shot generalization capability in comparison to 3D models. Furthermore, previous studies have demonstrated that self-supervised photometric consistency~\citep{mattersflow, vdba} enables the pre-trained flow estimator to effectively narrow the generalization gap across different data domains. Specifically, we employ a pre-trained 2D open-vocabulary segmentation model GroundedSAM~\citep{groundedsam} to derive a segmentation mask of movable objects. In addition, we use optical flow cues from an off-the-shelf 2D estimator~\citep{unimatch, cotracker} to offer effective supervision of pixel correspondence for joint geometry and motion optimization.

% \yx{This paragraph is a bit long, I think it can be deleted if you write the experimental results separately in the contribution}To evaluate the effectiveness of our proposed method, we conduct extensive experiments on both self-supervised 3D occupancy and occupancy flow prediction tasks. Compared with recent SOTA approaches with 2D or 3D supervision, our Let Occ Flow achieves competitive results on nuScenes~\citep{nuscenes} and KITTI~\citep{kitti} datasets. 

In summary, our main contributions are as follows:

1. We proposed Let Occ Flow, the first self-supervised method for jointly predicting 3D occupancy and occupancy flow, by integrating 2D optical flow cues into geometry and motion optimization.

2. We designed a novel temporal fusion module with BEV-based backward-forward attention for efficient temporal interaction. Furthermore, we proposed a two-stage optimization strategy and dynamic disentanglement scheme to mitigate the training instability and sample imbalance problem.

3. We conducted extensive experiments on various datasets with qualitative and quantitative analyses to show the competitive performance of our approach.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/teaser_lz2.pdf}
    \vspace{-0.4cm}
    \caption{\textbf{Let Occ Flow} introduces a novel self-supervised training paradigm for simultaneous prediction of 3D occupancy and occupancy flow. Unlike earlier studies that relied on expensive annotations for 3D occupancy flow, our method employs readily available 2D labels to train the occupancy flow network. Additionally, it uses 2D optical flows to facilitate dynamic decomposition and optimize both scene geometry and object motion jointly.}
    \label{fig:teaser}
    \vspace{-4mm}
\end{figure}

%===============================================================================
\section{Related Work}
\label{sec:relatedwork}

	% Citations can be made using either \textbackslash citep\{\} or \textbackslash citet\{\}, depending from the appropriateness. To avoid the citation moving to the next line, it is often a good practice to replace the space before with a tilde (\~{}) character.
	% Example 1: ``CoRL is the best conference ever~\citep{Gauss1857}.''
	% Example 2: ``\citet{Lagrange1788} proved, both theoretically and numerically, that CoRL is the best conference ever.''

\subsection{3D Occupancy Prediction}

Vision-centric 3D occupancy prediction has emerged as a promising method to perceive the surrounding environment. TPVFormer~\citep{tpvformer} introduces a tri-perspective view representation from multi-camera images. SurroundOcc~\citep{surroundocc} utilizes sparse LiDAR data to generate dense occupancy ground truth as supervision. Rather than using 3D labels, RenderOcc~\citep{renderocc} employs volume rendering to enable occupancy prediction from weak 2D semantic and depth labels. Recently, SimpleOccupancy~\citep{simpleocc}, OccNeRF~\citep{occnerf}, and SelfOcc~\citep{selfocc} propose a LiDAR-free self-supervised manner by photometric consistency. Despite the progress in static occupancy prediction, there has been comparatively less focus on occupancy flow prediction—a critical component for dynamic planning and navigation in autonomous driving. 

\subsection{Neural Radiance Field}
Reconstructing 3D scenes from 2D images remains a significant challenge in computer vision. Among the various approaches, Neural Radiance Field (NeRF)\citep{nerf} has gained increasing popularity due to its strong representational ability. To enhance training efficiency and improve rendering quality, several methods\citep{plenoxels, instantNGP, dvgo} have adopted explicit voxel-based representations. Additionally, some approaches~\citep{neus, spidr}  introduced NeRF into surface reconstruction by developing Signed Distance Function(SDF) representation. Further advancements~\citep{scenerf, behind, pixelsplat, mvsplat} have been made to facilitate scene-level sparse view reconstruction by conditioning NeRF on image features, laying the groundwork for generalizable NeRF architectures. 


\subsection{Scene Flow}
Scene flow enables autonomous systems to perceive motion in highly dynamic environments by offering dense motion estimation for each point in the scene.  FlowNet3D~\citep{flownet3d} introduced deep-learning to estimate scene flow when trained solely on synthetic data. NSFP~\citep{nsfp} optimizes a neural network to estimate the scene flow with expensive per-timestep optimization. Unlike previous methods that estimate correspondence between two input frames, some approaches proposed to combine scene flow prediction with vision-based occupancy network~\citep{occnet, viewformer}, while they rely heavily on complete 3D occupancy and flow annotations. Our proposed approach addresses this gap by being the first work to jointly predict 3D occupancy and occupancy flow in a self-supervised manner, establishing a new direction for future research in this field.

%===============================================================================
\section{Method}
\label{sec:method}

The overall framework is shown in Figure \ref{fig:pipeline}. In Sec.\ref{sec:encoder}, we first extract 3D volume features $V$ from multi-view temporal sequences with 2D-to-3D feature encoder. To capture the geometry and motion information, we employ an attention-based temporal fusion module and utilize a 3D refine module to ensure effective spatial-temporal interaction. Next in Sec.\ref{sec:render}, we construct the volumetric SDF and flow field using two MLP decoders and perform differentiable rendering to optimize the network with 2D labels in a self-supervised manner. Finally in Sec.\ref{sec:flow}, we illustrate a flow-oriented two-stage training strategy and dynamic disentanglement scheme for joint geometry and motion optimization.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\textwidth, keepaspectratio]{figure/pipeline_occflow3.pdf}
    \vspace{-0.5cm}
    \caption{\textbf{The overall architecture of Let Occ Flow}. We employ deformable-attention layers to integrate multi-view image input into TPV representation. The temporal fusion module utilizes BEV-based backward-forward attention to fuse temporal feature volumes. The 3D Refine Module further aggregates spatial features and upsample the fused volume into a high-solution representation. Then we apply two separate MLP decoders to construct volumetric SDF and flow fields, and finally perform self-supervised occupancy flow learning utilizing reprojection consistency, optical flow cues, and optional LiDAR ray supervision via differentiable rendering.
    }
    \label{fig:pipeline}
    \vspace{-3mm}
\end{figure*}

\subsection{Problem Formulation}
We aim to provide a unified framework for joint prediction of 3D occupancy $O_{t}$ and occupancy flow $F_{t}$ of the surrounding scenes at timestep $t$ using a temporal sequence of multi-view camera inputs. Formally, our prediction task is represented as:
\begin{equation}
    O_{t}, \, F_{t} = \mathcal{G}(I_{t-k},I_{t-k+1},...,I_{t})
    \label{setup}
\end{equation}

where $\mathcal{G}$ is a neural network, $I_{t}$ represents $N$-view images $\{I_{t}^{1},I_{t}^{2},...,I_{t}^{N}\}$ at timestamp $t$. $O_{t} \in \mathbb{R}^{H \times W \times Z}$ denotes the 3D occupancy at timestamp $t$, representing the occupied probability of each 3D volume grid with the value between 0 and 1. And $F_{t} \in \mathbb{R}^{H \times W \times Z \times 2}$ denotes the occupancy flow at timestamp $t$, representing the motion vector of each grid in the horizontal direction of 3D space. 

\subsection{2D-to-3D Encoder}
\label{sec:encoder}

\textbf{2D-to-3D Feature Encoder.} Following existing 3D occupancy methods~\citep{selfocc, tpvformer}, we utilize TPV to effectively construct a unified representation from multi-view image input, which pre-define a set of queries in the three axis-aligned orthogonal planes:
\begin{equation}
    T = \{T^{HW},T^{ZH}, T^{WZ}\}, \quad
    T^{HW} \in \mathbb{R}^{H \times W \times C}, \,
    T^{ZH} \in \mathbb{R}^{Z \times H \times C}, 
    T^{WZ} \in \mathbb{R}^{W \times Z \times C} \,
    \label{tpv}
\end{equation}
where $H, W, Z$ denote the resolution of the three planes and $C$ represents the feature dimension. We can integrate multi-view multi-scale image features $F$ extracted from the 2D encoder backbone~\citep{convnet} into triplane using deformable cross-attention~\citep{deformable} (DAttn) and feed forward network (FFN):
\begin{equation}
    T^{p_i} = FFN(DAttn(DAttn(T^{p_i},\{T^{p_j}\}_{p_j \in P-\{p_{i}\}}), F)), \quad p_i \in P=\{HW, ZH, WZ\}
    \label{tpv_da}
\end{equation}

Then we construct a full-scale 3D feature volume $V$ by broadcasting each TPV plane along the corresponding orthogonal direction and aggregating them by summation up~\citep{tpvformer}.

\textbf{Temporal Fusion.} To effectively capture temporal geometry and object motion, we design a temporal fusion module to enhance the scene representation further. Previous approaches~\citep{renderocc, fbocc} utilize a residual block of convolution networks to fuse concatenated temporal volume features. However, it is hard for the convolution module to align the volume features of moving objects due to the inherent local receptive field. In contrast, the attention module has been proven to have the ability to capture long-distance dependencies~\citep{bevformer}. Additionally, compared with voxel-based fusion, BEV-based temporal interaction is more computationally efficient without accuracy degradation~\citep{viewformer}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth, keepaspectratio]{figure/temporal_fusion2.pdf}
    \vspace{-0.6cm}
    \caption{\textbf{Architecture of temporal fusion module}. The temporal fusion module consists of ego-motion alignment and temporal feature aggregation. While ego-motion alignment is employed in voxel space to align temporal feature volumes, BEV-based temporal feature aggregation leverages deformable attention with a backward-forward process to achieve temporal interaction.}
    \label{fig:temporal_fusion}
    \vspace{-5mm}
\end{figure}

Specifically, our temporal fusion module integrates historical feature volume into the current frame. As depicted in \autoref{fig:temporal_fusion}, this module comprises two main components: ego-motion alignment in voxel space and a Backward-Forward Attention Module (BFAM) in BEV space. To compensate for ego-motion, we first apply feature warping by transforming historical feature volumes to the current frame, according to the relative pose in ego coordinate:
\begin{equation}
    \hat{V}_{t_i} = \left\langle V_{t_i}, T_{t}^{t_i} \cdot P_{t} \right\rangle, \quad t_i \in \{t-k,t-k+1,...,t-1\}
    \label{alignment}
\end{equation}

where $\hat{V}_{t_i} \in \mathbb{R}^{H \times W \times Z \times C}$ is the aligned feature volume in the current local ego coordinate. $P_t \in \mathbb{R}^{H \times W \times Z \times 3}$ denotes the predefined reference points of current feature volume, $T_{t}^{t_i}$ is the ego pose transformation matrix from $t$ to $t_i$, and $\left\langle \cdot,\cdot \right\rangle$ indicates the linear interpolation operator.

Inspired by prior works~\citep{occformer, henet}, we compress the aligned feature volume $\hat{V}_t$ into a series of BEV slices $B_t \in \mathbb{R}^{H \times W \times C} $ along the z-axis and employ deformable attention~\citep{deformable} (DAttn) between these BEV slices in the horizontal direction. To effectively capture overall information in the vertical dimension, we derive a global BEV feature $B_g$ using an average pooling operator and integrate it into the BEV slices. Furthermore, we employ a Backward-Forward Attention Module (BFAM) to enhance the interaction between temporal BEV features:
\begin{equation}
    B_{t_j} = B_{t_j} + \beta \cdot DAttn(B_{t_j}, \{B_{t_i}, B_{t_j}\})
\end{equation}

where $B_{t_i}, B_{t_j}$ represents the BEV features at adjacent frames $t_i, t_j$, and $\beta$ is a learnable scale factor. In the backward process, $t_j=t_i-1$, while in the forward process, $t_j=t_i+1$.

After BFAM, we recover the fused feature volume $\tilde{V}$ by merging fused BEV slices, and utilize the BEV-Volume Fusion module to achieve interaction between fused global BEV features $\tilde{B_g}$ and fused feature volume $\tilde{V}$ for the final feature volume $\tilde{V}^{\prime}$:
\begin{equation}
    \tilde{V}^{\prime}=\tilde{V}+\sigma(conv (\tilde{V})) \cdot unsqueeze(\tilde{B_g},-1)
\end{equation}
where $conv$ is a $1\times1$ convolution module and $\sigma$ is a sigmoid function.

\textbf{3D Refine Module.} Following the acquisition of the final fused feature volume $\tilde{V}^{\prime}$, we utilize a residual 3D convolution network to further aggregate spatial features and subsequently upsample it to refined feature volume $V_\mathit{refine}$ with high resolution using 3D deconvolutions.

\subsection{Rendering-Based Optimization}
\label{sec:render}

\textbf{Rendering Strategy.} Given refined feature volume $V_\mathit{refine}$, we employ two separate MLP $\{\Theta_s, \Theta_f\}$ to construct volumetric SDF field $\mathcal{S}$ and volumetric flow field $\mathcal{F}$:
\begin{equation}
  \mathcal{S} = \Theta_s(V_\mathit{refine}), \quad \mathcal{F} = \Theta_f(V_\mathit{refine})
\end{equation}

During training, we employ a rendering-based strategy to concurrently optimize the 3D occupancy and occupancy flow without 3D annotations. Following~\citep{simpleocc, selfocc}, we utilize SDF for geometric representation, with occlusion-aware rendering as NeuS\citep{neus}. Details are shown in the supplementary.

\textbf{Rendering-Based Supervision.} Inspired by~\citep{simpleocc, occnerf, selfocc, scenerf}, we utilize a reprojection photometric loss for effective optimization of the volumetric SDF field:
\begin{equation}
    \mathcal{L}_{reproj}(x) = \sum_{i=1}^{N}w_i\mathcal{L}_{photo}(\left\langle I_t, x \right\rangle, \left\langle I_{t+1}, K T^{-1} T_{t}^{t+1} (T K^{-1} [x, d_i]+f_i)\right\rangle)
\end{equation}
% \begin{equation}
%     \mathcal{L}_{reproj}(x) = \sum_{i=1}^{N}w_i \Vert ( I_t(x),  I_{t+1}( K T^{-1} T_{t}^{t+1} (T K^{-1} [x, d_i]+f_i)) \Vert
% \end{equation}

where $N$ denotes the number of points sampled along the ray, $x$ is the sampled pixel on the current image, $T_{t}^{t+1}$ represents the transformation matrix from timestamp $t$ to $t+1$ in ego coordinate, $K$ and $T$ are the intrinsic and extrinsic parameters of cameras, respectively. Additionally, $w_i$, $d_i$, and $f_i$ denote the weight, depth, and flow of $i^{th}$ sampled point. For the photometric loss $\mathcal{L}_{photo}$, we utilize the combination of L1 and D-SSIM loss, following monodepth~\citep{monodepth}.

Though photometric loss is sufficient for geometric supervision, optimizing object motion jointly remains a significant challenge. Therefore, we incorporate optical flow cues from an off-the-shelf flow estimator~\citep{unimatch, cotracker} to offer an additional source of supervision for geometry and motion estimation. 
% \begin{equation}
%     \label{eq:flow}
%     \mathcal{L}_{flow}(x) = \sum_{i=1}^{N}w_i \Vert \left\langle O_{t \rightarrow t+1}, x \right\rangle, KT_{t}^{t+1}(T_{C}^{E}d_iK^{-1}x+f_i)-x\Vert_1
% \end{equation}
\begin{equation}
    \label{eq:flow}
    \mathcal{L}_{flow}(x) = \sum_{i=1}^{N}w_i \Vert \left\langle O_{t \rightarrow t+1}, x \right\rangle, K T^{-1} T_{t}^{t+1}(T K^{-1}[x, d_i]+f_i)-x\Vert_1
\end{equation}
where $O_{t \rightarrow t+1}$ represents the estimated forward flow map from frame $t$ to $t+1$.

% In addition to photometric supervision, we could use extra LiDAR supervision to enhance the geometry, making our approach comparable to those with 3D labels as supervision. To accomplish this, we independently generate rays from the LiDAR measurement to ensure an effective sampling rate in regions with sufficient geometric observations, thereby avoiding occlusion problems from camera extrinsic. Furthermore, we implement a Scale-Invariant loss $\mathcal{L}_{range}$~\citep{silog} between rendered ranges and LiDAR measurements to mitigate the global scene scale influence effectively.

When LiDAR is available, we could combine LiDAR supervision to enhance the geometry. Specifically, we first independently generate rays from the LiDAR measurement to ensure an effective sampling rate in regions with sufficient geometric observations, thereby avoiding occlusion problems from camera extrinsic. Furthermore, we implement a Scale-Invariant loss $\mathcal{L}_{range}$~\citep{silog} between rendered ranges and LiDAR measurements to mitigate the global scene scale influence.


\textbf{SDF Field Regularization.} Due to the explicit physical interpretation of SDF representation, regularization can be effectively applied to the volumetric SDF field to prevent over-fitting with limited supervision. Initially, an eikonal term $\mathcal{L}_{eik}=(1-\Vert \left \langle \nabla\mathcal{S}, \bm{p} \right \rangle)\Vert_2)^2$ is employed for each sample point along camera and LiDAR rays to promote the establishment of a valid SDF field, where $\nabla\mathcal{S}$ denotes the pre-computed gradient field of the volumetric SDF grid. Additionally, we also utilize a Hessian loss $\mathcal{L}_{H}$ on the second-order derivatives of the SDF grid, following the approach of SelfOcc~\citep{selfocc}. Furthermore, an edge-aware smoothness loss $\mathcal{L}_{smooth}$ is employed following monodepth2~\citep{monodepth} to enforce neighborhood consistency of rendered depths and flows. 

\subsection{Flow-Oriented Optimization}
\label{sec:flow}

Due to the training instability caused by the inherent ambiguities in jointly optimizing geometry and motion without ground truth labels, and the sample imbalance problem of moving objects and the static background, it becomes imperative to employ an effective flow-oriented optimization strategy. 

\textbf{Two Stage Optimization.} To tackle the training instability challenge, we introduce a two-stage optimization strategy. Initially, we optimize the SDF field with the static assumption following the method proposed by SelfOcc~\citep{selfocc} to generate a coarse geometric prediction. In the second stage, we jointly optimize the volumetric SDF and flow field with extra 2D optical flow supervision. 

\textbf{Dynamic Disentanglement.} To effectively regularize the motion in static regions and solve the sample imbalance problem, we propose to conduct dynamic disentanglement using dynamic optical flow $f_x^{d}$, which is subtracted by flow cues $f_x^{opt}$ and static flow $f_x^{s}$ computed by rendered depth $d$:
% \begin{equation}
%     f_x^{d} = f_x^{opt} - f_x^{s}=\left\langle O_{t \rightarrow t+1}, x \right\rangle - (KT_{t}^{t+1}T_{C}^{E}dK^{-1}x - x)
% \end{equation}
\begin{equation}
    f_x^{d} = f_x^{opt} - f_x^{s}=\left\langle O_{t \rightarrow t+1}, x \right\rangle - (K T^{-1} T_{t}^{t+1} T K^{-1}[x, d] - x)
\end{equation}

\begin{wrapfigure}{r}{7cm}%靠文字内容的右侧
\centering
\vspace{-6mm}
\includegraphics[width=0.5\textwidth]{figure/dynamic_mask2.pdf}
\label{fig:dynamic-mask}
\vspace{-6mm}
\caption{Our effective dynamic disentanglement scheme provides accurate dynamic mask for joint geometry and motion optimization.}
\vspace{-6mm}
\end{wrapfigure}

To mitigate incorrect decomposition caused by inaccurate depth estimation in background regions(eg.sky and thin structure), we leverage the zero-shot open-vocabulary 2D semantic segmentation model, Grounded-SAM~\citep{groundedsam}, to extract binary masks for movable foreground objects. With flow error mask thresholded by dynamic flow $f_x^d$, we could get an accurate dynamic mask for scene decomposition. Then we can regularize the volumetric flow field by minimizing the rendered flow map in static regions: $\mathcal{L}_{dreg} = \Vert \sum_{m}^{M_{s}} \sum_i^N w_i f_i \Vert_1$.

Compared to the static background, dynamic objects such as cars or pedestrians account for a small proportion in driving scenes but hold significant importance for driving perception and planning. To address the imbalance caused by moving objects, we employ a scale factor to adjust the flow loss of dynamic rays based on their occurrence.
\begin{equation}
    \mathcal{L}_{flow} = \mathcal{L}_{flow}^{s} + \gamma \mathcal{L}_{flow}^{d}, \quad \gamma = min(M_{all}/M_{d}, thre)
\end{equation}

where $\mathcal{L}_{flow}^{s}$ and $\mathcal{L}_{flow}^{d}$ denote the static and dynamic parts of the flow loss $\mathcal{L}_{flow}$ calculated by \autoref{eq:flow}, while $M_{all}$ and $M_{d}$ represent the number of all sampled rays and dynamic rays, and $thre$ is a threshold hyperparameter.

% \textbf{Static flow supervision.} Since optical flow priors provide the pixel correspondence between adjacent frames, they could be used to effectively regularize the scene geometry. Specifically, we sample auxiliary frames based on the Gaussian distribution of the distance between the ego coordinates. Then we utilize the dynamic mask mentioned above to decouple the static part and then leverage static backward and forward flow to force the static geometry consistent.

\textbf{Static Flow Supervision.}  Since optical flow cues provide the pixel correspondence between adjacent frames, they could be used to supervise the scene geometry effectively. Specifically, we utilize the dynamic mask mentioned above to decouple the static regions and then leverage the forward static flow for geometry supervision. To effectively use the abundant training data in a self-supervised manner, we sample an auxiliary previous frame based on the Gaussian distribution of the distance between the ego coordinates to offer an additional backward flow for geometric supervision. 

Finally, our overall loss function is summarized as follows:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{reproj} + \lambda_{flow}\mathcal{L}_{flow} + \lambda_{range}\mathcal{L}_{range} + \lambda_{eik}\mathcal{L}_{eik} + \lambda_{H}\mathcal{L}_{H} + \lambda_{smooth}\mathcal{L}_{smooth} + \lambda_{dreg}\mathcal{L}_{dreg}
\end{equation}

\section{Experimental Results}
\label{sec:result}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth, keepaspectratio]{figure/results.pdf}
    \vspace{-0.5cm}
    \caption{\textbf{Visualization results for depth estimation, 3D occupancy and occupancy flow prediction on the KITTI~\citep{kitti} dataset.} Our method can predict visually appealing depth maps, fine-grained occupancy, and accurate dynamic decomposition and motion estimation.}
    \vspace{-4mm}
    \label{fig:vis}
\end{figure}

\subsection{Self-supervised 3D Occupancy Prediction}

We conduct experiments on 3D occupancy prediction using the  SemanticKITTI~\citep{semantickitti} dataset without LiDAR supervision and employ RayIoU~\citep{sparseocc} as evaluation metrics. We also evaluate the results of monocular depth estimation using Abs Rel, Sq Rel, RMSE, RMSE log as metrics.

As reported in \autoref{tab:occ-kitti}, our method sets the new
state-of-the-art for 3D occupancy prediction and depth estimation tasks without any form of 3D supervision compared with other supervised and self-supervised approaches. Thanks to our effective spatial-temporal feature aggregation and the integration of optical flow cues for supervision, our method greatly enhances the geometric representation capabilities, compared to other rendering-based methods~\citep{occnerf, selfocc, scenerf}.


\begin{table}[H] \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{ 3D occupancy prediction and depth estimation on SemanticKITTI~\citep{semantickitti} dataset. } MonoScene~\citep{monoscene} is trained with 3D supervision and cannot render monocular depth. We adapt the OccNeRF~\citep{occnerf} to the SemanticKITTI~\citep{semantickitti} dataset based on the official implementation.}
    
    \label{tab:occ-kitti}
    \begin{tabular}{ p{2.0cm}<{\centering} | p{1.0cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} | p{1.0cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{1.2cm}<{\centering} }
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{ Occupancy } & \multicolumn{4}{c}{ Depth } \\
        & IoU@1$\uparrow$ & IoU@2$\uparrow$ & IoU@4$\uparrow$ & RayIoU$\uparrow$ & Abs Rel$\downarrow$ & Sq Rel$\downarrow$ & RMSE$\downarrow$ & RMSE log$\downarrow$ \\
        \hline 
        MonoScene~\citep{monoscene} & 26.00 & 36.50 & 49.09 & 37.19 & - & - & - & - \\
        \hline 
        SceneRF~\citep{scenerf} & 20.65 & 35.74 & 56.35 & 37.58 & 0.146 & 1.048 & 5.240 & 0.241 \\
        OccNeRF~\citep{occnerf} & 23.22 & 40.17 & 62.57 & 41.99 & 0.132 & 1.011 & 5.497 & 0.233 \\
        SelfOcc~\citep{selfocc} & 23.13 & 35.38 & 50.31 & 36.27 & 0.152 & 1.306 & 5.386 & 0.245\\
        \textbf{Ours} & \textbf{28.62} & \textbf{45.60} & \textbf{66.95} & \textbf{47.06} & \textbf{0.117} & \textbf{0.817} & \textbf{4.816} & \textbf{0.215} \\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

\subsection{Self-supervised Occupancy Flow Prediction}

We conduct occupancy flow prediction on the KITTI-MOT~\citep{kitti} and nuScenes~\citep{nuscenes} datasets. To compare with the OccNeRF*~\citep{occnerf} and RenderOcc*~\citep{renderocc}, we add a concatenation\&conv temporal fusion module and an occupancy flow head to the original model with extra 2D optical flow labels as supervision. To compare with OccNet~\citep{occnet}, we use the official implementation to reproduce the results with GT 3D occupancy flow labels from OpenOcc~\citep{occnet} as supervision. 
% For the KITTI dataset, we used Unimatch~\citep{unimatch} to generate pseudo optical flow. As the 3D occupancy flow ground-truth data for nuScenes is only available at 2Hz keyframes and is challenging for optical flow estimation, we employed a tracking-based model~\citep{cotracker} on non-keyframe sequences to obtain pseudo optical flow. 
% put it in the supplementary materials

Due to the absence of occupancy flow annotations, we report the occupancy flow evaluation metrics on the KITTI-MOT dataset~\citep{kitti} using LiDAR-projected depths and generated flow labels. More details are presented in the supplementary materials. On the nuScenes~\citep{nuscenes} dataset, with annotated occupancy flow ground truth, we report the RayIOU~\citep{sparseocc} and mAVE metrics as OccNet~\citep{occnet}.

\begin{table}[H] 
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{ Self-supervised occupancy flow prediction on the KITTI-MOT~\citep{kitti} dataset.} } 
    \label{tab:flow-kitti}
    \begin{tabular}{ p{4cm}<{\centering} | p{0.5cm}<{\centering} p{0.6cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{1.0cm}<{\centering} p{1.2cm}<{\centering}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c}{ Occupancy Flow }  \\
        & DE$\downarrow$ & EPE$\downarrow$ & DE\_FG$\downarrow$ & EPE\_FG$\downarrow$ & D1\_5\%$\downarrow$ & F1\_10\%$\downarrow$ & SF1\_10\%$\downarrow$ \\
        \hline 
        OccNeRF*~\citep{occnerf} (w/o LiDAR) & 3.547 & 6.986 & 7.976 & 10.445 & 0.204 & 0.272 & 0.306\\
        \textbf{Ours (w/o LiDAR)} & 3.431 & 3.529 & 6.429 & 7.635 & 0.215 & 0.084 & 0.118 \\
        \hline
        OccNeRF*~\citep{occnerf} (w/ LiDAR) & 2.667 & 8.131 & 4.040 & 11.284 & \textbf{0.137} & 0.309 & 0.326\\
        \textbf{Ours (w/ LiDAR)} & \textbf{2.610} & \textbf{3.488} & \textbf{3.106} & \textbf{7.510} & 0.154 & \textbf{0.083} & \textbf{0.105} \\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

\begin{table}[H] 
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{ Occupancy flow prediction on the nuScenes~\citep{nuscenes} dataset.} For experiments using 2D labels as supervision, we use extra LiDAR ray supervision for occupancy flow prediction here.} 
    \label{tab:flow-nus}
    \begin{tabular}{ p{2.8cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{1.cm}<{\centering} p{1.cm}<{\centering} p{1.cm}<{\centering} p{1.cm}<{\centering} p{1.cm}<{\centering} }
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{Supervision} & \multicolumn{5}{c}{Occupancy Flow} \\
        & 3D & 2D & IOU@1$\uparrow$ & IOU@2$\uparrow$ & IOU@4$\uparrow$ & RayIOU$\uparrow$ & mAVE$\downarrow$  \\
        \hline 
        OccNet~\citep{occnet} & $\checkmark$ & & \textbf{29.28} & \textbf{39.68} & \underline{50.02} & \underline{39.66} & 1.61 \\
        \hline
        OccNeRF*~\citep{occnerf} & & $\checkmark$ & 16.62 & 29.25 & 49.17 & 31.68 & \underline{1.59} \\
        RenderOcc*~\citep{renderocc} & & $\checkmark$ & 20.27 & 32.68 & 49.92 & 36.67 & 1.63 \\
        \textbf{Ours} & & $\checkmark$ & \underline{25.49} & \underline{39.66} & \textbf{56.30} & \textbf{40.48} & \textbf{1.45} \\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

We report the results of occupancy flow prediction in \autoref{tab:flow-kitti} and \autoref{tab:flow-nus}. Compared to other rendering-based methods~\citep{occnerf, renderocc}, our approach performs much better on both KITTI-MOT~\citep{kitti} and nuScenes~\citep{nuscenes} dataset, owing to our effective temporal fusion module and flow-oriented optimization strategy. And compared with 3D supervised OccNet~\citep{occnet}, our approach achieves comparable performance on nuScenes~\citep{nuscenes}, validating the effectiveness of our self-supervised training paradigm. 

\subsection{Ablation Study}
We systematically conduct comprehensive ablation analyses on the temporal fusion module, optimization strategy, and static flow supervision to validate the effectiveness of every component of our method. All experiments are trained for 16 epochs, and without LiDAR supervision by default.

\begin{table}[H] 
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{Temporal fusion module ablation on KITTI-MOT~\citep{kitti} dataset.} } 
    \label{tab:ablation-fusion}
    \begin{tabular}{ p{3cm}<{\centering} | p{0.6cm}<{\centering} p{0.6cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} p{1.0cm}<{\centering} | p{0.8cm}<{\centering}}
        \toprule
        Temporal Fusion Module & DE$\downarrow$ & EPE$\downarrow$ & DE\_FG$\downarrow$ & EPE\_FG$\downarrow$ & D1\_5\%$\downarrow$ & F1\_10\%$\downarrow$ & SF1\_10\%$\downarrow$ & Params.$\downarrow$\\
        \hline 
        Concatenation\&3D Conv. & 3.515 & 3.638 & 6.423 & 7.743 & 0.223 & 0.090 & 0.126 & 11.39M\\
        BEV Pool\&Forward Attn. & 3.600 & 3.763 & \textbf{6.339} & 7.971 & 0.228 & 0.091 & 0.124 & \underline{5.21M} \\
        Ours  & \textbf{3.431} & \textbf{3.529} & 6.429 & \textbf{7.635} & \textbf{0.215} & \textbf{0.084} & \textbf{0.118} & 6.62M\\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

\begin{table}[H] 
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{Optimization strategy ablation on KITTI-MOT~\citep{kitti} dataset.} Since the absence of two-stage optimization brings instability during training, we use extra LiDAR ray supervision here. }
    \label{tab:ablation-reg}
    \begin{tabular}{ p{2.0cm}<{\centering} p{2.0cm}<{\centering} | p{0.5cm}<{\centering} p{0.6cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{1.0cm}<{\centering} p{1.2cm}<{\centering}}
        \toprule
        Two Stage Optimization & Dynamic Disentanglement & DE$\downarrow$ & EPE$\downarrow$ & DE\_FG$\downarrow$ & EPE\_FG$\downarrow$ & D1\_5\%$\downarrow$ & F1\_10\%$\downarrow$ & SF1\_10\%$\downarrow$ \\
        \hline 
        & & 3.760 & 4.403 & 4.194 & 8.853 & 0.258 & 0.121 & 0.152\\
        $\checkmark$ & & 3.064 & 3.633 & 3.600 & 7.966 & 0.191 & 0.089 & 0.114 \\
         $\checkmark$ & $\checkmark$ & \textbf{2.610} & \textbf{3.488} & \textbf{3.106} & \textbf{7.510} & \textbf{0.154} & \textbf{0.083} & \textbf{0.105}\\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

\begin{table}[H] 
    \scriptsize
    \renewcommand{\arraystretch}{1.2}
    \centering
    \vspace{-2mm}
    \caption{\textbf{Static flow supervision ablation on KITTI-MOT~\citep{kitti} dataset.}}
    \label{tab:ablation-flow}
    \begin{tabular}{ p{2.0cm}<{\centering} p{2.0cm}<{\centering} | p{0.5cm}<{\centering} p{0.6cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{0.9cm}<{\centering} p{1.0cm}<{\centering} p{1.2cm}<{\centering}}
        \toprule
        Backward Static Flow Supervision & Forward Static Flow Supervision & DE$\downarrow$ & EPE$\downarrow$ & DE\_FG$\downarrow$ & EPE\_FG$\downarrow$ & D1\_5\%$\downarrow$ & F1\_10\%$\downarrow$ & SF1\_10\%$\downarrow$ \\
        \hline 
        & & 6.715 & 4.128 & 6.598 & 8.160 & 0.239 & 0.099 & 0.149\\
        & $\checkmark$ & 3.495 & 3.614 & 6.510 & 7.987 & 0.217 & \textbf{0.084} & 0.123 \\
        $\checkmark$ & $\checkmark$ & \textbf{3.431} & \textbf{3.529} & \textbf{6.429} & \textbf{7.635} & \textbf{0.215} & \textbf{0.084} & \textbf{0.118} \\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}

\textbf{Temporal Fusion.} We report the results of different temporal fusion settings in \autoref{tab:ablation-fusion}. Our proposed method achieves the best results. Compared to the 3D Convolution module, our method achieves better performance with lower memory cost due to our effective BEV-based backward-forward attention mechanism and the efficient temporal interaction between adjacent frames, rather than relying on global 3D convolution. Additionally, Our method effectively incorporates local and global information on the height dimension compared to the BEV-only attention module.

\textbf{Optimization Strategy.} We investigate the effect of our optimization strategy in \autoref{tab:ablation-reg}. It is shown that both two-stage optimization and dynamic disentanglement scheme benefit mitigating the impact of the ambiguities for joint optimization of scene geometry and object motion.

\textbf{Static Flow Supervision.} We verify the effectiveness of static flow supervision in \autoref{tab:ablation-flow}. As reported, extra pixel correspondence priors from forward and backward static flow can effectively improve the quality of scene geometry, thus making occupancy flow better.

	
%===============================================================================

\section{Conclusion}
\label{sec:conclusion}

In this study, we introduced Let Occ Flow, the first self-supervised method for joint 3D occupancy and occupancy flow prediction using only camera input. Utilizing the effective temporal fusion module and flow-oriented optimization, our approach effectively captures dynamic object dependencies, thus enhancing both scene geometry and object motion. Furthermore, our method extends the differentiable rendering to the volumetric flow field and leverages 2D flow and semantic cues for dynamic disentanglement. Consequently, our work paves the way for future research into more efficient and accurate self-supervised learning frameworks in dynamic environment perception.

